GenGMM: Generalized Gaussian-Mixture-based Domain Adaptation Model for Semantic Segmentation

Domain adaptive semantic segmentation is the task of generating precise and dense predictions for an unlabeled target domain using a model trained on a labeled source domain. While significant efforts have been devoted to improving unsupervised domain adaptation for this task, it is crucial to note that many models rely on a strong assumption that the source data is entirely and accurately labeled, while the target data is unlabeled. In real-world scenarios, however, we often encounter partially or noisy labeled data in source and target domains, referred to as Generalized Domain Adaptation (GDA). In such cases, we suggest leveraging weak or unlabeled data from both domains to narrow the gap between them, resulting in effective adaptation. We introduce the Generalized Gaussian-mixture-based (GenGMM) domain adaptation model, which harnesses the underlying data distribution in both domains to refine noisy weak and pseudo labels. The experiments demonstrate the effectiveness of our approach.

==> related_work.tex <==
% \textbf{Unsupervised Domain Adaptation}

% UDA methods transfer knowledge from a labeled source domain to an unlabeled target domain \cite{wang2022cluster}. 
In recent UDA developments for semantic segmentation, 
% two primary approaches have emerged: adversarial learning training and self-training.
% Adversarial training addresses distribution shift at image-level \cite{hoffman2018cycada,li2019bidirectional}, feature-level \cite{chen2017deeplab, li2021t}, and output-level \cite{luo2019taking, melas2021pixmatch}. However, they may not ensure clear distinguishability among target domain classes \cite{long2018conditional}. 
% To address this, Wang et al. (2020) \cite{wang2020differential} and Zhang et al. (2019) \cite{zhang2019category} employed source category anchors, although anchor selection can be complex, and global category anchors based on unimodal distribution assumptions may overlook within-class variations.
% On the other hand, 
self-training approaches incorporate pseudo labels assigned to samples from the target domain to facilitate iterative training. The central concern in these techniques is how to achieve stable model training in the presence of noisy pseudo labels. 
Various strategies have been proposed, including dynamic threshold strategies \cite{zou2019confidence} and uncertainty estimation strategies \cite{zheng2019unsupervised}, to select high-quality pseudo labels.
Another area of research \cite{zhang2021prototypical} utilized distances to category prototypes to improve pseudo labels. However, these methods assume a single mode in the source domain's underlying distribution, neglecting within-class variations. The challenges of unimodality, noisy pseudo labels, and domain shift emphasize the need for further research in the field of UDA. 
% Most studies focus on introducing various strategies to refine the discriminative classifier outputs, ignoring the underlying distribution of source and target domain data. To address these challenges, we propose to incorporate the underlying distribution of source and target domain data using a Gaussian Mixture Model (GMM) as a generative model, in conjunction with a discriminative classifier, to enhance the performance of the UDA model.
% \noindent
% \textbf{Weakly Supervised Domain Adaptation}
On the other hand, Weakly Supervised Domain Adaptive Semantic Segmentation (WDASS) is a technique that simplifies the task of adapting to new data domains by incorporating less detailed target data annotations, referred to as weak labels. Previous methods \cite{paul2020domain,das2023urban} have experimented with various weak label types, such as image-level, point, and bounding box labels, and employed techniques like adversarial alignment, self-training, and boundary loss to enhance WDASS performance. However, despite the potential advantages of weak labels, these studies treat weak labels as supplementary information. Das et al. (2023)\cite{das2023weakly} tackled the challenge of aligning source and target features by utilizing weak labels by learning learning class prototypes.
Constructing these prototypes presents a considerable challenge. Moreover, these studies have primarily focused on scenarios where clean source data and weakly labeled target data are available. In real-world practical situations, however, we often encounter weakly labeled source and target data. 

